Speeding-up One-vs-All Training for Extreme Classification via Smart Initialization

In this paper we show that a simple, data dependent way of setting the initial vector can be used to substantially speed up the training of linear one-versus-all (OVA) classifiers in extreme multi-label classification (XMC). We discuss the problem of choosing the initial weights from the perspective of three goals. We want to start in a region of weight space a) with low loss value, b) that is favourable for second-order optimization, and c) where the conjugate-gradient (CG) calculations can be performed quickly. For margin losses, such an initialization is achieved by selecting the initial vector such that it separates the mean of all positive (relevant for a label) instances from the mean of all negatives -- two quantities that can be calculated quickly for the highly imbalanced binary problems occurring in XMC. We demonstrate a speedup of $\approx 3\times$ for training with squared hinge loss on a variety of XMC datasets. This comes in part from the reduced number of iterations that need to be performed due to starting closer to the solution, and in part from an implicit negative mining effect that allows to ignore easy negatives in the CG step. Because of the convex nature of the optimization problem, the speedup is achieved without any degradation in classification accuracy.

==> supplementarty/s-and-t/CmpIterDuration.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={iteration},
xmin=0, xmax=15,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=100000, ymax=1633853.15684273,
ymode=log,
ytick style={color=black},
width=0.5\linewidth,
xmajorgrids,
ymajorgrids
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,225321.983945527)
--(axis cs:0,344038.857314788)
--(axis cs:1,467390.949852621)
--(axis cs:2,475216.075525121)
--(axis cs:3,468783.445526141)
--(axis cs:4,462368.112873579)
--(axis cs:5,435858.042158368)
--(axis cs:6,447457.595297406)
--(axis cs:7,461423.60115509)
--(axis cs:8,514133.583313948)
--(axis cs:9,546779.918539638)
--(axis cs:10,542073.317565321)
--(axis cs:11,601149.19185384)
--(axis cs:12,442017.158545047)
--(axis cs:13,508669.774650955)
--(axis cs:14,435921.717121312)
--(axis cs:15,327000.727526457)
--(axis cs:16,332111.359276149)
--(axis cs:17,342266.767843426)
--(axis cs:18,312338.297761552)
--(axis cs:19,315131.293083833)
--(axis cs:20,325129.999961294)
--(axis cs:21,335365.986416007)
--(axis cs:22,308866.003533365)
--(axis cs:22,196366.996466635)
--(axis cs:22,196366.996466635)
--(axis cs:21,201532.013583993)
--(axis cs:20,221786.000038706)
--(axis cs:19,259769.706916167)
--(axis cs:18,238943.702238448)
--(axis cs:17,257998.660728003)
--(axis cs:16,264056.440723851)
--(axis cs:15,254575.772473543)
--(axis cs:14,208674.914457635)
--(axis cs:13,191181.853256022)
--(axis cs:12,218437.319715823)
--(axis cs:11,133719.970936858)
--(axis cs:10,195026.408413326)
--(axis cs:9,171858.408368612)
--(axis cs:8,167326.623440015)
--(axis cs:7,173946.153818385)
--(axis cs:6,168657.924557501)
--(axis cs:5,178424.383216487)
--(axis cs:4,163670.286495364)
--(axis cs:3,170218.963899043)
--(axis cs:2,167512.498754591)
--(axis cs:1,181066.399884813)
--(axis cs:0,225321.983945527)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,230920.071050038)
--(axis cs:0,328839.073436083)
--(axis cs:1,402543.066139806)
--(axis cs:2,436296.153688131)
--(axis cs:3,437049.087230496)
--(axis cs:4,450816.801958906)
--(axis cs:5,423600.747192884)
--(axis cs:6,430548.557607323)
--(axis cs:7,453965.584889622)
--(axis cs:8,514082.465435521)
--(axis cs:9,585343.583885191)
--(axis cs:10,611614.806271237)
--(axis cs:11,582948.578209273)
--(axis cs:12,621200.888578009)
--(axis cs:13,514811.472247193)
--(axis cs:14,344021.334664389)
--(axis cs:15,334524.237711563)
--(axis cs:16,357747.750338764)
--(axis cs:17,335833.308822927)
--(axis cs:18,320271.396460082)
--(axis cs:19,315956.336881059)
--(axis cs:20,317071.093348331)
--(axis cs:21,309508.256276514)
--(axis cs:22,261638.074567061)
--(axis cs:23,251150.873110634)
--(axis cs:24,258657.984520658)
--(axis cs:25,302847.997540852)
--(axis cs:25,165402.002459148)
--(axis cs:25,165402.002459148)
--(axis cs:24,227229.015479342)
--(axis cs:23,239763.126889366)
--(axis cs:22,249440.925432939)
--(axis cs:21,252206.143723486)
--(axis cs:20,259153.306651669)
--(axis cs:19,242340.463118942)
--(axis cs:18,292423.174968489)
--(axis cs:17,278181.941177073)
--(axis cs:16,266878.694105681)
--(axis cs:15,276921.048002722)
--(axis cs:14,244361.498668945)
--(axis cs:13,175468.992869086)
--(axis cs:12,143202.385931795)
--(axis cs:11,188415.256573336)
--(axis cs:10,157499.904920098)
--(axis cs:9,141830.388358448)
--(axis cs:8,156878.182177122)
--(axis cs:7,172685.256544157)
--(axis cs:6,175777.091953057)
--(axis cs:5,182211.002616654)
--(axis cs:4,165978.724767821)
--(axis cs:3,183515.989900356)
--(axis cs:2,183316.306545962)
--(axis cs:1,206750.609179024)
--(axis cs:0,230920.071050038)
--cycle;
\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:27,305929.561919148)
--(axis cs:27,306030.438080852)
--(axis cs:27,305929.561919148)
--(axis cs:27,305929.561919148)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,407778.519709028)
--(axis cs:0,596134.89484461)
--(axis cs:1,1562418.24322816)
--(axis cs:2,1243011.43686591)
--(axis cs:3,971615.935083091)
--(axis cs:4,727084.200876551)
--(axis cs:5,536246.978823235)
--(axis cs:6,420057.69188227)
--(axis cs:7,363965.25231529)
--(axis cs:8,342049.867636268)
--(axis cs:9,314630.135563075)
--(axis cs:10,304972.393400589)
--(axis cs:11,279398.205526391)
--(axis cs:12,271454.210969835)
--(axis cs:13,266397.126473243)
--(axis cs:14,265994.528303209)
--(axis cs:15,266585.583732921)
--(axis cs:16,267646.170417115)
--(axis cs:17,267427.768981258)
--(axis cs:18,276877.813781133)
--(axis cs:19,278255.970690076)
--(axis cs:20,278536.288515039)
--(axis cs:21,279434.376262393)
--(axis cs:22,280212.505682436)
--(axis cs:23,305201.696416096)
--(axis cs:24,239785.053737252)
--(axis cs:25,242208.951145721)
--(axis cs:25,213641.048854279)
--(axis cs:25,213641.048854279)
--(axis cs:24,208333.612929415)
--(axis cs:23,216020.58929819)
--(axis cs:22,222279.648163718)
--(axis cs:21,200356.290404274)
--(axis cs:20,195506.135727385)
--(axis cs:19,195910.775072636)
--(axis cs:18,202834.77337483)
--(axis cs:17,198184.061134572)
--(axis cs:16,193451.541957467)
--(axis cs:15,191385.318586124)
--(axis cs:14,191988.403120137)
--(axis cs:13,191374.102216985)
--(axis cs:12,190493.586525975)
--(axis cs:11,190818.136182996)
--(axis cs:10,178516.215356473)
--(axis cs:9,186664.722275215)
--(axis cs:8,185130.252405958)
--(axis cs:7,198415.333692074)
--(axis cs:6,213585.111509596)
--(axis cs:5,233879.669736189)
--(axis cs:4,293841.324369154)
--(axis cs:3,405121.363941665)
--(axis cs:2,645362.380088332)
--(axis cs:1,954762.894506272)
--(axis cs:0,407778.519709028)
--cycle;
\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:27,234887.540375166)
--(axis cs:27,234918.459624834)
--(axis cs:28,236524.351128075)
--(axis cs:29,294078.366652186)
--(axis cs:29,294001.633347814)
--(axis cs:29,294001.633347814)
--(axis cs:28,236455.648871925)
--(axis cs:27,234887.540375166)
--cycle;

\addplot [thick, color0]
table {%
0 284680.420630158
1 324228.674868717
2 321364.287139856
3 319501.204712592
4 313019.199684471
5 307141.212687428
6 308057.759927453
7 317684.877486737
8 340730.103376981
9 359319.163454125
10 368549.862989324
11 367434.581395349
12 330227.239130435
13 349925.813953488
14 322298.315789474
15 290788.25
16 298083.9
17 300132.714285714
18 275641
19 287450.5
20 273458
21 268449
22 252616.5
};
\addlegendentry{$t=-2$}
\addplot [thick, color0, opacity=0.2, dashed, forget plot]
table {%
0 344038.857314788
1 467390.949852621
2 475216.075525121
3 468783.445526141
4 462368.112873579
5 435858.042158368
6 447457.595297406
7 461423.60115509
8 514133.583313948
9 546779.918539638
10 542073.317565321
11 601149.19185384
12 442017.158545047
13 508669.774650955
14 435921.717121312
15 327000.727526457
16 332111.359276149
17 342266.767843426
18 312338.297761552
19 315131.293083833
20 325129.999961294
21 335365.986416007
22 308866.003533365
};
\addplot [thick, color0, opacity=0.2, dashed, forget plot]
table {%
0 225321.983945527
1 181066.399884813
2 167512.498754591
3 170218.963899043
4 163670.286495364
5 178424.383216487
6 168657.924557501
7 173946.153818385
8 167326.623440015
9 171858.408368612
10 195026.408413326
11 133719.970936858
12 218437.319715823
13 191181.853256022
14 208674.914457635
15 254575.772473543
16 264056.440723851
17 257998.660728003
18 238943.702238448
19 259769.706916167
20 221786.000038706
21 201532.013583993
22 196366.996466635
};
\addplot [thick, color1]
table {%
0 279879.572243061
1 304646.837659415
2 309806.230117047
3 310282.538565426
4 308397.763363363
5 302905.874904769
6 303162.82478019
7 313325.420716889
8 335480.323806321
9 363586.98612182
10 384557.355595668
11 385681.917391304
12 382201.637254902
13 345140.23255814
14 294191.416666667
15 305722.642857143
16 312313.222222222
17 307007.625
18 306347.285714286
19 279148.4
20 288112.2
21 280857.2
22 255539.5
23 245457
24 242943.5
25 234125
26 288808
27 305980
};
\addlegendentry{$t=-3$}
\addplot [thick, color1, opacity=0.2, dashed, forget plot]
table {%
0 328839.073436083
1 402543.066139806
2 436296.153688131
3 437049.087230496
4 450816.801958906
5 423600.747192884
6 430548.557607323
7 453965.584889622
8 514082.465435521
9 585343.583885191
10 611614.806271237
11 582948.578209273
12 621200.888578009
13 514811.472247193
14 344021.334664389
15 334524.237711563
16 357747.750338764
17 335833.308822927
18 320271.396460082
19 315956.336881059
20 317071.093348331
21 309508.256276514
22 261638.074567061
23 251150.873110634
24 258657.984520658
25 302847.997540852
26 nan
27 306030.438080852
};
\addplot [thick, color1, opacity=0.2, dashed, forget plot]
table {%
0 230920.071050038
1 206750.609179024
2 183316.306545962
3 183515.989900356
4 165978.724767821
5 182211.002616654
6 175777.091953057
7 172685.256544157
8 156878.182177122
9 141830.388358448
10 157499.904920098
11 188415.256573336
12 143202.385931795
13 175468.992869086
14 244361.498668945
15 276921.048002722
16 266878.694105681
17 278181.941177073
18 292423.174968489
19 242340.463118942
20 259153.306651669
21 252206.143723486
22 249440.925432939
23 239763.126889366
24 227229.015479342
25 165402.002459148
26 nan
27 305929.561919148
};
\addplot [thick, color2]
table {%
0 501956.707276819
1 1258590.56886722
2 944186.908477119
3 688368.649512378
4 510462.762622852
5 385063.324279712
6 316821.401695933
7 281190.293003682
8 263590.060021113
9 250647.428919145
10 241744.304378531
11 235108.170854694
12 230973.898747905
13 228885.614345114
14 228991.465711673
15 228985.451159522
16 230548.856187291
17 232805.915057915
18 239856.293577982
19 237083.372881356
20 237021.212121212
21 239895.333333333
22 251246.076923077
23 260611.142857143
24 224059.333333333
25 227925
26 256548
27 234903
28 236490
29 294040
30 265900
};
\addlegendentry{$t=-1$}
\addplot [thick, color2, opacity=0.2, dashed, forget plot]
table {%
0 596134.89484461
1 1562418.24322816
2 1243011.43686591
3 971615.935083091
4 727084.200876551
5 536246.978823235
6 420057.69188227
7 363965.25231529
8 342049.867636268
9 314630.135563075
10 304972.393400589
11 279398.205526391
12 271454.210969835
13 266397.126473243
14 265994.528303209
15 266585.583732921
16 267646.170417115
17 267427.768981258
18 276877.813781133
19 278255.970690076
20 278536.288515039
21 279434.376262393
22 280212.505682436
23 305201.696416096
24 239785.053737252
25 242208.951145721
26 nan
27 234918.459624834
28 236524.351128075
29 294078.366652186
30 nan
};
\addplot [thick, color2, opacity=0.2, dashed, forget plot]
table {%
0 407778.519709028
1 954762.894506272
2 645362.380088332
3 405121.363941665
4 293841.324369154
5 233879.669736189
6 213585.111509596
7 198415.333692074
8 185130.252405958
9 186664.722275215
10 178516.215356473
11 190818.136182996
12 190493.586525975
13 191374.102216985
14 191988.403120137
15 191385.318586124
16 193451.541957467
17 198184.061134572
18 202834.77337483
19 195910.775072636
20 195506.135727385
21 200356.290404274
22 222279.648163718
23 216020.58929819
24 208333.612929415
25 213641.048854279
26 nan
27 234887.540375166
28 236455.648871925
29 294001.633347814
30 nan
};
\end{axis}
\end{tikzpicture}


==> supplementarty/s-and-t/CmpObjective.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\nextgroupplot[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={iteration},
xmajorgrids,
xmin=0, xmax=15,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={loss},
ymajorgrids,
ymin=1, ymax=17347.5830648474,
ymode=log,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,23.773591047037)
--(axis cs:0,3057.0838787395)
--(axis cs:1,634.257611016826)
--(axis cs:2,387.903508264016)
--(axis cs:3,304.023697704823)
--(axis cs:4,273.306598429468)
--(axis cs:5,265.190978453316)
--(axis cs:6,321.968075480796)
--(axis cs:7,569.18193830871)
--(axis cs:8,1166.29257719957)
--(axis cs:9,1861.80822905486)
--(axis cs:10,2266.61594688163)
--(axis cs:11,1545.13409526611)
--(axis cs:12,933.303677623899)
--(axis cs:13,465.6747879276)
--(axis cs:14,182.46275054949)
--(axis cs:15,57.6841471778243)
--(axis cs:16,51.2456184663802)
--(axis cs:17,33.8623735198234)
--(axis cs:18,29.1048828351508)
--(axis cs:19,32.8034994531956)
--(axis cs:20,37.8633914372835)
--(axis cs:21,37.8071451743216)
--(axis cs:22,37.7787063034767)
--(axis cs:22,13.5836891979277)
--(axis cs:22,13.5836891979277)
--(axis cs:21,13.5839217965344)
--(axis cs:20,13.5840082929212)
--(axis cs:19,13.1507858911891)
--(axis cs:18,10.1371044747243)
--(axis cs:17,10.970139054883)
--(axis cs:16,7.68453560831422)
--(axis cs:15,6.16392254053754)
--(axis cs:14,4.93202378267766)
--(axis cs:13,6.98876651556853)
--(axis cs:12,12.9854273704227)
--(axis cs:11,15.261239365638)
--(axis cs:10,24.5122375805026)
--(axis cs:9,21.3966518672748)
--(axis cs:8,15.3344536037399)
--(axis cs:7,9.04569427762197)
--(axis cs:6,7.02503946534578)
--(axis cs:5,6.82359895868298)
--(axis cs:4,6.89703889707973)
--(axis cs:3,7.02632841625568)
--(axis cs:2,7.78188565482169)
--(axis cs:1,10.0755759141829)
--(axis cs:0,23.773591047037)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,27.9909755398677)
--(axis cs:0,2506.05761152852)
--(axis cs:1,664.88611748671)
--(axis cs:2,395.799012699683)
--(axis cs:3,305.014150662512)
--(axis cs:4,273.729022359643)
--(axis cs:5,262.353557754239)
--(axis cs:6,286.573462376636)
--(axis cs:7,461.859765105079)
--(axis cs:8,997.803592773233)
--(axis cs:9,1753.58766841726)
--(axis cs:10,2418.18185439566)
--(axis cs:11,2586.74564247489)
--(axis cs:12,1921.21096908906)
--(axis cs:13,830.506366017674)
--(axis cs:14,202.103892812258)
--(axis cs:15,163.763930580008)
--(axis cs:16,54.7813907774548)
--(axis cs:17,41.9506065722177)
--(axis cs:18,42.8350301848155)
--(axis cs:19,44.6028796113512)
--(axis cs:20,44.5175258827426)
--(axis cs:21,44.496125017661)
--(axis cs:22,30.8337330765643)
--(axis cs:23,30.7741353759734)
--(axis cs:24,30.6843064915994)
--(axis cs:25,30.6708480927245)
--(axis cs:26,30.651555779919)
--(axis cs:27,30.654681993729)
--(axis cs:27,30.6244898649936)
--(axis cs:27,30.6244898649936)
--(axis cs:26,30.6322578645666)
--(axis cs:25,18.2229035374089)
--(axis cs:24,18.261685982886)
--(axis cs:23,18.3397748163628)
--(axis cs:22,18.3413275570679)
--(axis cs:21,12.366760920396)
--(axis cs:20,12.3715583899634)
--(axis cs:19,12.4050733184196)
--(axis cs:18,12.586547806322)
--(axis cs:17,8.60193087319925)
--(axis cs:16,9.28943051743241)
--(axis cs:15,5.12662595933527)
--(axis cs:14,5.8018462378152)
--(axis cs:13,7.20517448766934)
--(axis cs:12,12.235196293203)
--(axis cs:11,17.9991701968823)
--(axis cs:10,20.6050807387077)
--(axis cs:9,16.9172722669952)
--(axis cs:8,10.5831151548683)
--(axis cs:7,7.03573630797369)
--(axis cs:6,6.36169804514018)
--(axis cs:5,6.80825102081395)
--(axis cs:4,6.91963523409955)
--(axis cs:3,7.12329583477637)
--(axis cs:2,8.092566724146)
--(axis cs:1,11.2093503805284)
--(axis cs:0,27.9909755398677)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,588.846911721123)
--(axis cs:0,16521.6565989764)
--(axis cs:1,1637.65608153987)
--(axis cs:2,661.599387610599)
--(axis cs:3,475.48556882805)
--(axis cs:4,385.391120019314)
--(axis cs:5,328.245466799782)
--(axis cs:6,293.263276806706)
--(axis cs:7,268.878941599788)
--(axis cs:8,247.881228522603)
--(axis cs:9,222.574255761049)
--(axis cs:10,177.666273768093)
--(axis cs:11,128.265489135817)
--(axis cs:12,83.4932479482398)
--(axis cs:13,51.408733816474)
--(axis cs:14,35.996714236551)
--(axis cs:15,31.1587050055765)
--(axis cs:16,35.3454023932944)
--(axis cs:17,44.1552177060698)
--(axis cs:18,46.7925182642555)
--(axis cs:19,48.0722940927122)
--(axis cs:20,55.7570033396319)
--(axis cs:21,79.4435288304939)
--(axis cs:22,107.657106935267)
--(axis cs:23,208.828472921037)
--(axis cs:24,24.9295397462075)
--(axis cs:25,24.8762548668398)
--(axis cs:26,24.9212503271258)
--(axis cs:27,24.9082912129071)
--(axis cs:28,24.8655532859607)
--(axis cs:29,24.8635860466122)
--(axis cs:29,24.8317187240007)
--(axis cs:29,24.8317187240007)
--(axis cs:28,24.8353786793924)
--(axis cs:27,24.8745439374083)
--(axis cs:26,24.8944808589)
--(axis cs:25,15.7672812252166)
--(axis cs:24,15.7681311524138)
--(axis cs:23,16.2338741546994)
--(axis cs:22,8.59426751696835)
--(axis cs:21,7.30584592843718)
--(axis cs:20,5.48024427793125)
--(axis cs:19,5.12982154592368)
--(axis cs:18,3.90430839172056)
--(axis cs:17,3.18551219991616)
--(axis cs:16,3.12728155686211)
--(axis cs:15,3.19228684462392)
--(axis cs:14,3.66629564268209)
--(axis cs:13,4.82773208507616)
--(axis cs:12,6.00836820449079)
--(axis cs:11,6.8398421721665)
--(axis cs:10,7.22162598074144)
--(axis cs:9,7.4351926345449)
--(axis cs:8,7.69148853115434)
--(axis cs:7,8.13347187893556)
--(axis cs:6,8.7759714830641)
--(axis cs:5,9.75628936281105)
--(axis cs:4,11.3115955328804)
--(axis cs:3,14.1802418876495)
--(axis cs:2,23.9416092677443)
--(axis cs:1,65.9011965580084)
--(axis cs:0,588.846911721123)
--cycle;

\addplot [thick, color0]
table {%
0 269.588319349416
1 79.9406699305699
2 54.9419761786446
3 46.2187228988266
4 43.4166585563259
5 42.538886732332
6 47.5587892700604
7 71.7540647091499
8 133.732791092735
9 199.590737562429
10 235.711324704008
11 153.559959884941
12 110.087906330957
13 57.0481582964156
14 29.9985103823984
15 18.8563149905032
16 19.8443639322348
17 19.2736853310634
18 17.1767062623931
19 20.7699734662978
20 22.6789907906454
21 22.6620675005218
22 22.6533486426669
};
\addplot [thick, color0, opacity=0.2, dashed, forget plot]
table {%
0 3057.0838787395
1 634.257611016826
2 387.903508264016
3 304.023697704823
4 273.306598429468
5 265.190978453316
6 321.968075480796
7 569.18193830871
8 1166.29257719957
9 1861.80822905486
10 2266.61594688163
11 1545.13409526611
12 933.303677623899
13 465.6747879276
14 182.46275054949
15 57.6841471778243
16 51.2456184663802
17 33.8623735198234
18 29.1048828351508
19 32.8034994531956
20 37.8633914372835
21 37.8071451743216
22 37.7787063034767
};
\addplot [thick, color0, opacity=0.2, dashed, forget plot]
table {%
0 23.773591047037
1 10.0755759141829
2 7.78188565482169
3 7.02632841625568
4 6.89703889707973
5 6.82359895868298
6 7.02503946534578
7 9.04569427762197
8 15.3344536037399
9 21.3966518672748
10 24.5122375805026
11 15.261239365638
12 12.9854273704227
13 6.98876651556853
14 4.93202378267766
15 6.16392254053754
16 7.68453560831422
17 10.970139054883
18 10.1371044747243
19 13.1507858911891
20 13.5840082929212
21 13.5839217965344
22 13.5836891979277
};
\addplot [thick, color1]
table {%
0 264.852784213785
1 86.330420212447
2 56.5953171174373
3 46.6122948261735
4 43.5213164749805
5 42.2630911954446
6 42.697702928735
7 57.0045920829367
8 102.761229674719
9 172.237974995818
10 223.21924726757
11 215.775983545318
12 153.317948484381
13 77.3559518090077
14 34.2428928415899
15 28.9750999603841
16 22.5585443518743
17 18.9962158816695
18 23.2194994607211
19 23.522372154854
20 23.4680883506744
21 23.4578971772293
22 23.780908270385
23 23.7569087417454
24 23.6716532957083
25 23.6413177763897
26 30.6419053030425
27 30.6395822104603
};
\addplot [thick, color1, opacity=0.2, dashed, forget plot]
table {%
0 2506.05761152852
1 664.88611748671
2 395.799012699683
3 305.014150662512
4 273.729022359643
5 262.353557754239
6 286.573462376636
7 461.859765105079
8 997.803592773233
9 1753.58766841726
10 2418.18185439566
11 2586.74564247489
12 1921.21096908906
13 830.506366017674
14 202.103892812258
15 163.763930580008
16 54.7813907774548
17 41.9506065722177
18 42.8350301848155
19 44.6028796113512
20 44.5175258827426
21 44.496125017661
22 30.8337330765643
23 30.7741353759734
24 30.6843064915994
25 30.6708480927245
26 30.651555779919
27 30.654681993729
};
\addplot [thick, color1, opacity=0.2, dashed, forget plot]
table {%
0 27.9909755398677
1 11.2093503805284
2 8.092566724146
3 7.12329583477637
4 6.91963523409955
5 6.80825102081395
6 6.36169804514018
7 7.03573630797369
8 10.5831151548683
9 16.9172722669952
10 20.6050807387077
11 17.9991701968823
12 12.235196293203
13 7.20517448766934
14 5.8018462378152
15 5.12662595933527
16 9.28943051743241
17 8.60193087319925
18 12.586547806322
19 12.4050733184196
20 12.3715583899634
21 12.366760920396
22 18.3413275570679
23 18.3397748163628
24 18.261685982886
25 18.2229035374089
26 30.6322578645666
27 30.6244898649936
};
\addplot [thick, color2]
table {%
0 3119.0906470996
1 328.517115724549
2 125.856084596462
3 82.1127297078132
4 66.025665249373
5 56.5902620256317
6 50.7313527740547
7 46.7645090890499
8 43.664351893393
9 40.6802466447029
10 35.8195390610373
11 29.6195155568879
12 22.3977270333815
13 15.7539707280079
14 11.488019696899
15 9.97334066824248
16 10.51356385934
17 11.8598897420102
18 13.5163760575411
19 15.7035757074233
20 17.4803317619149
21 24.0915375525711
22 30.4176589681809
23 58.2245236074814
24 19.8265542212335
25 19.8048202798113
26 24.9078619967369
27 24.8914118559237
28 24.8504614027475
29 24.8476472765424
30 24.8362636864164
};
\addplot [thick, color2, opacity=0.2, dashed, forget plot]
table {%
0 16521.6565989764
1 1637.65608153987
2 661.599387610599
3 475.48556882805
4 385.391120019314
5 328.245466799782
6 293.263276806706
7 268.878941599788
8 247.881228522603
9 222.574255761049
10 177.666273768093
11 128.265489135817
12 83.4932479482398
13 51.408733816474
14 35.996714236551
15 31.1587050055765
16 35.3454023932944
17 44.1552177060698
18 46.7925182642555
19 48.0722940927122
20 55.7570033396319
21 79.4435288304939
22 107.657106935267
23 208.828472921037
24 24.9295397462075
25 24.8762548668398
26 24.9212503271258
27 24.9082912129071
28 24.8655532859607
29 24.8635860466122
30 nan
};
\addplot [thick, color2, opacity=0.2, dashed, forget plot]
table {%
0 588.846911721123
1 65.9011965580084
2 23.9416092677443
3 14.1802418876495
4 11.3115955328804
5 9.75628936281105
6 8.7759714830641
7 8.13347187893556
8 7.69148853115434
9 7.4351926345449
10 7.22162598074144
11 6.8398421721665
12 6.00836820449079
13 4.82773208507616
14 3.66629564268209
15 3.19228684462392
16 3.12728155686211
17 3.18551219991616
18 3.90430839172056
19 5.12982154592368
20 5.48024427793125
21 7.30584592843718
22 8.59426751696835
23 16.2338741546994
24 15.7681311524138
25 15.7672812252166
26 24.8944808589
27 24.8745439374083
28 24.8353786793924
29 24.8317187240007
30 nan
};
\end{axis}
\end{tikzpicture}


==> supplementarty/s-and-t/CmpShift.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\end{axis}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{Shift};
\end{tikzpicture}

